Power to the Data Defenders: Human-Centered Disclosure Risk Calibration of Open Data

The open data ecosystem is susceptible to vulnerabilities due to disclosure risks. Though the datasets are anonymized during release, the prevalence of the release-and-forget model makes the data defenders blind to privacy issues arising after the dataset release. One such issue can be the disclosure risks in the presence of newly released datasets which may compromise the privacy of the data subjects of the anonymous open datasets. In this paper, we first examine some of these pitfalls through the examples we observed during a red teaming exercise and then envision other possible vulnerabilities in this context. We also discuss proactive risk monitoring, including developing a collection of highly susceptible open datasets and a visual analytic workflow that empowers data defenders towards undertaking dynamic risk calibration strategies.

==> sections/approach_dataset_development.tex <==
\section{Approach: Dataset Development}\label{section:dataset_development}

Open data portals contain a multitude of datasets on varying topics like economics, health, and others. However, they may not be relevant in information disclosure about human activity. On top of that, the problems discussed in the previous section press for an urgent need for a smaller subset of open datasets focused on disclosure risks. Hence we curated a seed set of datasets that contains a subset of the open datasets, which may be more susceptible to vulnerabilities related to disclosure. In this section, we discuss developing this dataset and the learning outcomes.

\subsection{Data collection}
Many open data portals are developed using frameworks/APIs like Socrata API~\cite{SocrataAPI}, CKAN API~\cite{CKANAPI}, DKAN API~\cite{DKANAPI}, etc. We selected the Socrata API as our source for the open datasets. Though other APIs could have served a similar purpose, we planned to start with Socrata and develop a generalizable approach that can help integrate the other publicly available APIs. 

First, we queried the list of all available data portals through Socrata Discovery API. From each of these data portals, we queried the metadata for all the data items available within them. Data items include datasets, maps, data dictionaries, etc. We filtered these results and created a list of $39,507$ datasets.
\subsection{Data analysis}
Manually analyzing all these datasets would be a difficult task for any analyst. Hence we developed a semi-automated program that filters datasets if they have some combinations of the known quasi-identifiers. Initially, we started with a list of the known quasi-identifiers like \textit{age}, \textit{sex}, \textit{race}, and \textit{age group}, to name a few, and the program selected the datasets with these attributes. After evaluating the attribute space of the selected datasets, we subsequently updated this list to include more such quasi-identifiers. This helped us to select a broader set of datasets that may be susceptible to disclosure risk through these quasi-identifiers.

Multiple iterations of this process led to the development of a set of about $5404$ datasets with some combination of the quasi-identifiers. We also manually verified the unselected datasets to check if we had missed any such vulnerable datasets. 
\subsection{Data curation}
After reducing the set of candidate datasets, the next step was to determine if these datasets relate to human objects and activity.
Hence, we started manually curating the metadata file to understand what each dataset pertains to. For each of the datasets, we opened them in their respective data portals and analyzed them to understand if they were related to human data subjects or not. We observed many such datasets with location attributes (like zip code, address, etc.). However, they do not necessarily relate to human beings, like \textit{datasets for street lamps}, \textit{building details}, etc. We dropped those datasets since they are irrelevant in the context of the privacy of the data subjects. 

Removing these datasets related to non-human objects, we curated a seed set of $426$ datasets of varying granularity. $151$ of these datasets were individual record-level~(e.g., records of people committing crimes) while the rest $275$ datasets were aggregated record-level~(e.g., college records) datasets~(Figure~\ref{figs:dataset_development}). We understand that a dataset collection like this should be continuously updated. However, we need more infrastructure to set up a method to fetch and update this collection regularly. Thus, we release a metadata file for this dataset collection as a contribution to this paper.


==> sections/deprecated/background.tex <==
\section{Background}\label{section:background}
Open datasets are those datasets that can be freely used, re-used, and redistributed by anyone~\cite{opendatadefinition}. The motivation behind creating open datasets is to promote transparency and accountability in public information, especially government data. It helps to democratize information instead of confining it within the data owners and a select few who can pay for it~\cite{kitchin2014towards}. Governments worldwide share these datasets through various open data portals like NYC Open Data~\cite{NYCOpenData}, Chicago Open Data~\cite{CityofChicagoOpenData}, Australian Capital Territory Open Data~\cite{ACTOpenData} etc., and are generally guided by the FAIR data principle~\cite{wilkinson2016fair}. This principle provides guidelines to improve the \textit{f}indability, \textit{a}ccessibility, \textit{i}nteroperability, and \textit{r}eusability of digital data. Findability is essential for the automatic discovery of datasets; hence metadata with a persistent and unique identifier is generally recommended. These principles state that these metadata should be accessible to all. However, they can be protected using proper authentication procedures in order to prevent unauthorized or malicious access. Open datasets can be interoperable by using similar vocabulary for the attributes and metadata, which again promotes their re-usability in different domains. All these factors make the open data ecosystem a prime choice for research.

But easy accessibility and findability can lead to more concerns. Due to their simple accessibility and findability, these open datasets are generally anonymized before release. Information theoretic guarantees like k-anonymity, l-diversity, t-closeness are generally applied to these datasets. These guarantees help to reduce the possible disclosure risks, i.e., the risk of sensitive information about the individuals mentioned in a dataset being disclosed. Still, joining two anonymized datasets using protected attributes can lead to the disclosure of sensitive information. There are multiple examples where these datasets become vulnerable to disclosure risk in the presence of other newly released datasets. Researchers were able to re-identify $91$\% of all the taxis running in NYC using the NYC taxi open data and a taxi medallion dataset~\cite{douriez2016anonymizing}. The sensitivity of the information contained in this dataset makes it prudent to protect it against all possible disclosures.

However, finding disclosures becomes quite challenging for data defenders since these disclosures can be a function of time. Datasets released at a later point in time may affect the previously released datasets. Data defenders face this quagmire since information about all the possible future datasets to be released is not available during the actual release of a dataset. Moreover, data defenders follow the practice of ``release-and-forget" where after the release of a dataset, almost no checks are done to ensure protection of these datasets against newly released datasets~\cite{rocher2019estimating}. In order to protect the open data ecosystem from disclosure risks, a collaboration between multiple stakeholders is the need of the hour. Hence, we choose these open datasets and plan to empower the data defenders and data subjects to inspect their privacy while joining them. 

%This ecosystem is motivated by the FAIR data principles, which aim to improve the findability, accessibility, interoperability and reusability of datasets. Governments worldwide release these datasets in order to improve accountability and transparency of public interest data. Thus, these open datasets may also contain sensitive information about citizens.

%The Open Data Charter was signed by the leaders of the G8 nations in 2013, leading to the increasing adoption of datasets that can be freely used, re-used, and redistributed by anyone, commonly referred to as \textit{open datasets}~\cite{opendatadefinition, Ourhisto94:online}. Though these are generally anonymized before release, joining two anonymized datasets using protected attributes can lead to the disclosure of sensitive information. In this context, \textit{direct identifiers} are those protected attributes that can directly link to and identify an individual from a dataset (like name, id, SSN), while \textit{quasi-identifiers} are those protected attributes that individually do not uniquely identify an individual but when combined with others, can identify an individual~(e.g., age, race, gender, location). 

%Quasi-identifier like the age of a person cannot point to a specific individual, but a combination of other quasi-identifiers like race, gender, location, job title, etc. can disclose the information about the individual since the presence of an individual of a certain age, gender, race in a particular location can be unique enough to identify the individual. 

%Privacy-preserving data publishing and mining research has developed a suite of anonymization methods~\cite{fung2010privacy} addressing the problem of linking among public and private datasets, for example, between Census data and hospital records. The most promising among those methods is the notion of differential privacy that has recently been adopted by the US Census. However, besides US Census data, which is just one of the sources of openly available data about people and their behavior, there are now a plethora of open data portals. The adoption of open data portals is a recent phenomenon, with the promise of transparency and utility as depicted by the FAIR principles~\cite{wilkinson2016fair}, and at the same time, with the need for adherence to emerging privacy laws~\cite{nouwens2020dark}. The unrestricted availability of open data~\cite{green2017open} naturally raises the question: what if datasets within the open data ecosystem are linked even without any other sensitive information from private datasets? Researchers have recently expressed the need to investigate privacy issues in open data portals. Lavrenovs and Podins showed how the privacy of passengers can be violated through the public transportation open data, released by the city municipal of Riga, Latvia\cite{lavrenovs2016privacy}. Recent studies have demonstrated how even heavily anonymized datasetscan be used to re-identify about $99\%$ of Americans~\cite{rocher2019estimating}. Re-identification or disclosure of sensitive information is a challenge that has been previously explored by multiple researchers\cite{de2015unique, de2013unique, zang2011anonymization}. Risk of re-identification can be considered as a temporal function which is dependent on the datasets available at the time of analysis. Sekara et al. have recently performed a study which shows that this risk varies over time for the re-identification using smartphone app usage dataset with publicly available information\cite{sekara2021temporal}. But, data owners often practice the ``release and forget" model where datasets, once released, are not analyzed further for potential privacy risks with respect to the newly released datasets\cite{ohm2009broken, rubinstein2016anonymization}. This may lead to inadvertent breach of privacy when new datasets are released which, when joined with the existing datasets, can leak sensitive information. Thus it is necessary for the data owners to proactively monitor the the risks of their datasets with respect to other datasets available through the various open data portals and keep checking on a regular basis. We developed the PRIVEE workflow and visualization interface with this specific goal of realizing a defender-in-the-loop analytical framework that can be privy to the disclosure risks or possibility of accidental leakage of sensitive information whenever new datasets are released. The target users of PRIVEE are mainly data custodians or data owners but even data subjects~\cite{bhattacharjee2020privacy} themselves can use the workflow to inspect how vulnerable their identity or personal information might be, in the presence of multiple, linked data sets. We use the concept of dataset joinability~\cite{miller2018making} in the presence of quasi-identifiers as a means for calibrating discloure risks that are communicated using interactive visualizations throughout the PRIVEE workflow. While we do find examples of visualization techniques for expressing disclosure risks of individual datasets~\cite{kao2017using,dasgupta2019}, visualizing disclosure risk among multiple datasets, with input from data defenders, is largely an open problem that we address in PRIVEE.

==> sections/deprecated/methods_old.tex <==
\section{Methods}\label{section:methods}
Addressing the problem of disclosure risks while joining open datasets can be challenging due to the need for research works highlighting the vulnerabilities with real-world disclosure examples. Hence, we used a two-prong approach where we first conducted an ethical hacking exercise to expose the vulnerabilities of the open data ecosystem. Then we developed a set of highly susceptible datasets based on our findings from this exercise. In this section, we discuss the methods used to discover these vulnerabilities of the open data ecosystem.
%In this section, we discuss three possible attack scenarios that we identified during this exercise.
\subsection{Red team approach}
In order to explore the vulnerabilities related to the open data ecosystem, we conducted a \textit{red-team exercise} with the help of researchers in data privacy and urban informatics. A red-team exercise can be generally defined as a structured process to better understand the capabilities and vulnerabilities of a system by viewing the problems through the lenses of an adversary~\cite{zenko2015red}. In this subsection, we discuss the different stages of this exercise.
\par \noindent \textbf{Quasi-identifiers and disclosures:} Red-team exercises generally follow the cyber kill chain. It starts with the initial reconnaissance step, where attackers try to find vulnerable entry points into any target system. Moreover, attackers used \textit{quasi-identifiers}~\cite{motwani2007efficient} like age, race, gender, and location to breach privacy by linking multiple datasets~\cite{sweeney2005privacy}. Inspired by this, we bootstrapped our red-teaming activity by searching for datasets with these known quasi-identifiers. During our initial exploration, analysis of these datasets led to interesting observations where some of the datasets have a highly skewed distribution of records across different categories of the quasi-identifiers.

\par \noindent \textbf{Disclosures through joining datasets:} These highly skewed datasets established that vulnerabilities exist in individual record-level datasets. However, this leads to an essential question of whether these datasets can be actually joined with other open datasets to expose sensitive information. Join is a fundamental operation that connects two or more datasets, and joinability is the measure to determine if two datasets are linkable by any number of join keys~\cite{dong2021efficient,chia2019khyperloglog}. When these \textit{join keys coincide with protected attributes} like age, race, location, etc., the outcome of the join can potentially reveal sensitive information about an individual or even disclose the individual's identity. As a next step in the red-teaming exercise, we randomly selected vulnerable pairs of datasets from multiple open data portals~\cite{NYCOpenData, KansasCityOpenData, DallasOpenData} and analyzed them for~\textit{joinability risks}, in terms of what kind of sensitive information may be leaked by these joins. 

\textbf{Disclosures through transitive joins:} Inspired by the disclosure examples while joining two datasets and the concept of transitive dependency in databases~\cite{codd1972further}, we explored the concept that two datasets, which have no shared attributes between them, can still be joined if they have shared attributes with a third dataset. We experimented with different permutations of dataset joins in order to find an example of transitive disclosure. Though we did not find any examples of transitive disclosure at this stage, this can be an interesting field of research that can further strengthen the inspection of disclosure risk in open datasets. Hence, in another current work, we focus on assessing the risk of disclosure through transition (or \textit{transitive disclosure risk}) in open datasets to prevent the disclosure of sensitive information about an individual or a group of individuals.
\subsection{Data development approach}\label{section:dataset_development}
%\section{Approach: Dataset Development}\label{section:dataset_development}

Open data portals contain a multitude of datasets on varying topics like economics, health, and others. However, they may not be relevant in information disclosure about human activity. On top of that, the examples observed during the red teaming exercise press for an urgent need for a smaller subset of open datasets focused on disclosure risks. Hence we curated a seed set of datasets that contains a subset of the open datasets, which may be more susceptible to vulnerabilities related to disclosure. In this subsection, we discuss developing this dataset and the learning outcomes.

%\subsection{Data collection}
\par \noindent \textbf{Data collection:}
Many open data portals are developed using frameworks/APIs like Socrata API~\cite{SocrataAPI}, CKAN API~\cite{CKANAPI}, DKAN API~\cite{DKANAPI}, etc. We selected the Socrata API as our source for the open datasets. Though other APIs could have served a similar purpose, we planned to start with Socrata and develop a generalizable approach that can help integrate the other publicly available APIs. 

First, we queried the list of all available data portals through Socrata Discovery API. From each of these data portals, we queried the metadata for all the data items available within them. Data items include datasets, maps, data dictionaries, etc. We filtered these results and created a list of $39,507$ datasets.
%\subsection{Data analysis}
\par \noindent \textbf{Data analysis:}
Manually analyzing all these datasets would be a difficult task for any analyst. However, during our red teaming exercise, we understood that quasi-identifiers' presence could be an indicator of possible disclosures. Hence we developed a semi-automated program that filters datasets if they have some combinations of the known quasi-identifiers. Initially, we started with a list of the known quasi-identifiers like \textit{age}, \textit{sex}, \textit{race}, and \textit{age group}, to name a few, and the program selected the datasets with these attributes. After evaluating the attribute space of the selected datasets, we subsequently updated this list to include more such quasi-identifiers. This helped us to select a broader set of datasets that may be susceptible to disclosure risk through these quasi-identifiers.
\begin{figure}
 \begin{center}
\includegraphics[width=\columnwidth]{datasetDevelopment.pdf}
%\vspace{-6mm}
 \caption{\textbf{Dataset development:} The dataset development process starts with over $216,000$ data resources from $496$ data portals. After a few filtering steps, it consists of $426$ highly susceptible datasets with different levels of granularities and distribution of quasi-identifiers.}
 \label{figs:dataset_development}
 \end{center}
\vspace{-8mm}
\end{figure}
Multiple iterations of this process led to the development of a set of about $5404$ datasets with some combination of the quasi-identifiers. We also manually verified the unselected datasets to check if we had missed any such vulnerable datasets. 
%\subsection{Data curation}
\par \noindent \textbf{Data curation:}
After reducing the set of candidate datasets, the next step was to determine if these datasets relate to human objects and activity.
Hence, we started manually curating the metadata file to understand what each dataset pertains to. For each of the datasets, we opened them in their respective data portals and analyzed them to understand if they were related to human data subjects or not. We observed many such datasets with location attributes (like zip code, address, etc.). However, they do not necessarily relate to human beings, like \textit{datasets for street lamps}, \textit{building details}, etc. We dropped those datasets since they are irrelevant in the context of the privacy of the data subjects. 

Removing these datasets related to non-human objects, we curated a seed set of $426$ datasets of varying granularity. $151$ of these datasets were individual record-level~(e.g., records of people committing crimes) while the rest $275$ datasets were aggregated record-level~(e.g., college records) datasets~(Figure~\ref{figs:dataset_development}). We understand that a dataset collection like this should be continuously updated. However, we need more infrastructure to set up a method to fetch and update this collection regularly. Thus, we release a metadata file for this dataset collection as a contribution to this paper.


==> sections/problem.tex <==
\section{Problem}\label{section:problem}
In order to explore the vulnerabilities related to the open data ecosystem, we conducted a \textit{red-team exercise} with the help of researchers in data privacy and urban informatics. A red-team exercise can be generally defined as a structured process to better understand the capabilities and vulnerabilities of a system by viewing the problems through the lenses of an adversary~\cite{zenko2015red}. In this section, we discuss three possible attack scenarios that we identified during this exercise.

\subsection{Attack through vulnerable entry points}
Red-team exercises generally follow the cyber kill chain. It starts with the initial reconnaissance step, where attackers try to find vulnerable entry points into any target system. Moreover, attackers used \textit{quasi-identifiers}~\cite{motwani2007efficient} like age, race, gender, and location to breach privacy by linking multiple datasets~\cite{sweeney2005privacy}. Inspired by this, we bootstrapped our red-teaming activity by searching for datasets with these known quasi-identifiers. During our initial exploration, analysis of these datasets led to interesting observations where some of the datasets have a highly skewed distribution of records across different categories of the quasi-identifiers.

For example, the dataset \textit{Whole Person Care Demographics 2}~\cite{WholePersonDemographics2:online} from the \textit{County of San Mateo Datahub} portal~\cite{SMCDatahub:online} had only one record for a 26-year-old female of the Hawaiian race. This can lead to identity disclosure and leak of sensitive information when joined with other datasets. Another dataset \textit{Demographics for Public Health, Policy, and Planning}~\cite{Demographics:online}, from the same data portal, had only seven records for age $19$. However, out of these seven people, only one person was male. This individual can be identified since other identifying attributes like race, language, and city were also present. This may also lead to attribute disclosure if other similar datasets are exploited.
 
The dataset \textit{Overdose Information Network Data CY January 2018 - Current Monthly County State Police}~\cite{Overdose41:online} from the \textit{Pennsylvania Open Data}~\cite{OpenDataPA} portal had only few records for the race American Indian/Alaskan Native. However, out of these few people, only one was of Hispanic ethnicity. This dataset also contained location attributes, thus making it easy to pinpoint an individual with these attributes. When joined with other publicly available information, this information may lead to identity and attribute disclosure for this individual.

Thus, datasets with vulnerable entry points can be exploited to reveal sensitive information about an human data subjects. The presence of such datasets in the open data ecosystem can be considered a warning sign that calls for the development of a method that acts as the trusted informer for data custodians and informs them of potential disclosures in a proactive manner.

\subsection{Attack exploiting dataset joins}
The previous attack scenario established that vulnerabilities exist in individual record-level datasets. However, this leads to an essential question of whether these datasets can be actually joined with other open datasets to expose sensitive information. Join is a fundamental operation that connects two or more datasets, and joinability is the measure to determine if two datasets are linkable by any number of join keys~\cite{dong2021efficient,chia2019khyperloglog}. When these \textit{join keys coincide with protected attributes} like age, race, location, etc., the outcome of the join can potentially reveal sensitive information about an individual or even disclose the individual's identity.

As a next step in the red-teaming exercise, we randomly selected vulnerable pairs of datasets from multiple open data portals~\cite{NYCOpenData, KansasCityOpenData, DallasOpenData} and analyzed them for~\textit{joinability risks}, in terms of what kind of sensitive information may be leaked by these joins. Several iterations of the selection of joinable pairs and join keys led to the discovery of disclosure between the datasets \textit{Juvenile Arrests} and \textit{Adult Arrests} from the \textit{Fort Lauderdale Police Open Data Portal}~\cite{FortLauderdaleOpenData:online}. We observed that two individuals, aged $15$ and $21$, mentioned separately in these datasets, were involved in the same incident of larceny on $20$\textsuperscript{th} March $2018$, at the Coral Ridge Country Club Estate, Fort Lauderdale.
%(DO NOT DELETE) Amy observed that for the incident id $341803044797$ and caseid $341803044797$, the Adult Arrests dataset lists the age as $21$ while the Juvenile Arrests dataset lists the age as $15$ (Joined on incident id and case id.) More sensitive information like this can also be observed in other common records where the \textit{incidentid} and \textit{caseid} are $341807108870$ and it discloses the fact that two people, aged $17$ and $21$, were involved in a theft of motor vehicle (VEH THEFT-GRAND THEFT OF MOTOR VEHICLE) on $8$\textsuperscript{th} of July, $2018$.
%(DO NOT DELETE)She also joins the dataset pair \textit{Arrest} and \textit{Citations} on the unique identifier \textit{case\_id} and observes $2760$ common records. For example, a $28$ year old black male was arrested for larceny on $26$\textsuperscript{th} September $2021$ at NW $10$\textsuperscript{th} Ave, was also cited for disobeying stop/yield sign and driving while license is suspended at NW $9$\textsuperscript{th} Street, around $3$ miles away from the arrest location(case\_id: $342109159680$). Other dataset pairs like \textit{Citations} and \textit{Juvenile Arrests} have $90$ common records when joined on the unique identifier \textit{case\_id}, where a $17$-year old white male was first charged with disobeying red light and was later arrested for possession of cannabis over $20$ grams on $4$\textsuperscript{th} August, $2015$, both at N Federal Hwy, Fort Lauderdale.(case id: 341508122414)
This can be an example of identity disclosure by joining two open datasets. Further investigation revealed other examples where two individuals, aged $17$ and $21$, mentioned separately in these datasets, were involved in the same incident of motor vehicle theft on $8$\textsuperscript{th} of July, $2018$. The presence of linking attributes like \textit{case id} between datasets \textit{Adult Arrests} and \textit{Citations} helped to reveal an incident where a 28-year-old black male who was arrested for larceny on $26$\textsuperscript{th} September $2021$ at NW $10$\textsuperscript{th} Ave, Fort Lauderdale, was also cited for disobeying stop/yield sign and driving while license is suspended at NW $9$\textsuperscript{th} Street, just around $3$ miles away from the arrest location. A similar incident was also observed while joining datasets \textit{Citations} and \textit{Juvenile Arrests} on the linking attribute \textit{case id}. In this incident, a 17-year-old white male was first charged with disobeying a red light. He was later arrested for possession of cannabis over $20$ grams on $4$\textsuperscript{th} August, $2015$, both at N Federal Hwy, Fort Lauderdale.

We repeated this exercise and found other examples where dataset joins ultimately led to disclosures. In another example, two datasets, namely \textit{Electronic Police Report $2016$} and \textit{Electronic Police Report $2015$} from \textit{New Orleans Open Data} portal~\cite{NewOrleans:online}, were joined on quasi-identifiers like \textit{location}, \textit{victim age}, \textit{offender age}, \textit{victim race}, \textit{victim gender}, and \textit{offender gender}. On inspection of the joined records, we observed that a 22-year-old black male was charged with attempted robbery with a gun against a 27-year-old white male at 6XX Tchoupitoulas St on $13$\textsuperscript{th} July $2015$ at $01$:$00$ hrs and again on $30$\textsuperscript{th} April $2016$ at $03$:$00$ hrs with attempted simple robbery. This is an example of identity disclosure even when \textit{masking techniques} are used on the address. Another observation from these joined records revealed an incident where a runaway female juvenile of age $17$ was reported at 85XX Dinkins St on $26$\textsuperscript{th} February $2015$, and the same incident was closed through a supplemental report one and half years later on $7$\textsuperscript{th} December $2016$. Incidents like these may be rare; hence, identifying the individuals from these records may not be difficult.

We also observed such examples across other open data portals. Datasets \textit{APD Arrests Dataset by Neighborhood}, and \textit{APD Field Interview Cards Dataset by Neighborhood} from the \textit{Albany Police Department}~\cite{AlbanyPolice:online} were joined on the attributes \textit{age}, \textit{race}, \textit{sex}, and \textit{neighborhoodxy}. We observed that a $28$-year old white male was interviewed by the police in the Washington Park neighborhood at $09$:$08$ hrs on $1$\textsuperscript{st} December, $2020$ and was later arrested for trespassing on enclosed property at $12$:$32$ hrs. This leads to attribute disclosure for the individual arrested as the arrest details are revealed. Joining other datasets like \textit{APD Arrests Dataset by Patrol Zone} and \textit{APD Field Interview Cards Dataset by Neighborhood} from the same data portal revealed similar incidents where a $26$-year old black female was interviewed at $11$:$23$ hrs on $11$\textsuperscript{th} December, $2020$ and was later arrested at $21$:$25$ hrs for "assault with intent to cause physical injury". In another example, joining datasets \textit{APD Field Interview Cards Dataset by Neighborhood} and \textit{APD Traffic Citations by Neighborhood} on a broader set of attributes like \textit{age}, \textit{sex}, \textit{neighborhoodxy} and  \textit{date} led to another interesting observation related to a police incident. We observed that a $23$-year old male was stopped for a field interview on $23$\textsuperscript{rd} January, $2021$ at $2$:$45$ am. Since field interviews are usual routine stop and search activities by the police, this may seem a regular incident. However, the other dataset informed that an individual of the same age and gender received a citation on the same date and at the exact location at $2$:$48$ am, just $3$ minutes after the incident from the first dataset. Since both these records seem to belong to the same person, this is a possible identity disclosure, and it was discovered using a combination of date and quasi-identifiers like location coordinates, age, and gender.

\subsection{Attack through transitive dataset join}
Inspired by these examples and the concept of transitive dependency in databases~\cite{codd1972further}, we explored the concept that two datasets, which have no shared attributes between them, can still be joined if they have shared attributes with a third dataset. We experimented with different permutations of dataset joins in order to find an example of transitive disclosure. Though we did not find any examples of transitive disclosure at this stage, this can be an interesting field of research that can further strengthen the inspection of disclosure risk in open datasets. Hence, in another current work, we focus on assessing the risk of disclosure through transition (or \textit{transitive disclosure risk}) in open datasets to prevent the disclosure of sensitive information about an individual or a group of individuals.
\begin{figure}
 \begin{center}
\includegraphics[width=\columnwidth]{datasetDevelopment.pdf}
%\vspace{-6mm}
 \caption{\textbf{Dataset development:} The dataset development process starts with over $216,000$ data resources from $496$ data portals. After a few filtering steps, it consists of $426$ highly susceptible datasets with different levels of granularities and distribution of quasi-identifiers.}
 \label{figs:dataset_development}
 \end{center}
%\vspace{-2mm}
\end{figure}
